Study of alternative locations for the SPS Beam Dump Facility

As part of the main focus of the BDF Working Group in 2021, this document reports on the study of alternative locations and possible optimisation that may accompany the reuse of existing facilities with the aim of significantly reducing the costs of the facility. Building on the BDF/SHiP Comprehensive Design Study (CDS), the assessment rests on the generic requirements and constraints that allow preserving the physics reach of the facility by making use of the $4\times 10^{19}$ protons per year at 400\,GeV that are currently not exploited at the SPS and for which no existing facility is compatible. The options considered involve the underground areas TCC4, TNC, and ECN3. Recent improvements of the BDF design at the current location (referred to as `TT90-TCC9-ECN4') are also mentioned together with ideas for yet further improvements. The assessments of the alternative locations compiled the large amount of information that is already available together with a set of conceptual studies that were performed during 2021. The document concludes with a qualitative comparison of the options, summarising the associated benefits and challenges of each option, such that a recommendation can be made about which location is to be pursued. The most critical location-specific studies required to specify the implementation and cost for each option are identified so that the detailed investigation of the retained option can be completed before the end of 2022.

==> notes.tex <==


Additional points/studies:

- Interference between ECN3 and EHN2: The distance between the beamline in TCC8 and TT84 is about 30m. The muon flux is very forward directed. In the strongest version of the muon shield, the core of the muon plumes after the muon shield are at about 60mrad, the shower drops off completely at about 80mrad. The outer edge of the plume will only cross the axis of the EHN2 facility beyond 300m, so even after the Compass surface building.

- Hadron flux in 1203 CV room

- Interference with T4 target / M2 beamline while constructing?
